Exploring the Frontiers of Softmax: Provable Optimization, Applications in Diffusion Model, and Beyond

The softmax activation function plays a crucial role in the success of large language models (LLMs), particularly in the self-attention mechanism of the widely adopted Transformer architecture. However, the underlying learning dynamics that contribute to the effectiveness of softmax remain largely unexplored. As a step towards better understanding, this paper provides a theoretical study of the optimization and generalization properties of two-layer softmax neural networks, providing theoretical insights into their superior performance as other activation functions, such as ReLU and exponential. Leveraging the Neural Tangent Kernel (NTK) framework, our analysis reveals that the normalization effect of the softmax function leads to a good perturbation property of the induced NTK matrix, resulting in a good convex region of the loss landscape. Consequently, softmax neural networks can learn the target function in the over-parametrization regime. To demonstrate the broad applicability of our theoretical findings, we apply them to the task of learning score estimation functions in diffusion models, a promising approach for generative modeling. Our analysis shows that gradient-based algorithms can learn the score function with a provable accuracy. Our work provides a deeper understanding of the effectiveness of softmax neural networks and their potential in various domains, paving the way for further advancements in natural language processing and beyond.

==> 59_impact.tex <==
\section{Societal Impact}\label{sec:impact}

Our work focuses on improving our understanding of the learning dynamics behind the success of softmax activation functions. Our paper is purely theoretical (a mathematics problem), and thus, we foresee no immediate negative ethical impact. 

The study applies these theoretical insights to the scoring function learning of the diffusion model, showing that the gradient algorithm can learn the scoring function with provable precision, further confirming the effectiveness and wide applicability of the softmax network. This achievement deepens the scientific understanding of the high efficiency of softmax networks and lays a solid foundation for the future development of natural language processing and other fields, heralding the transition from the Pre-LLM era to the LLM era.
